Effective Quotation: relating approaches to language-integrated query

Language-integrated query techniques have been explored in a number of different language designs. We consider two different, type-safe approaches employed by Links and F#. Both approaches provide rich dynamic query generation capabilities, and thus amount to a form of heterogeneous staged computation, but to date there has been no formal investigation of their relative expressiveness. We present two core calculi Eff and Quot, respectively capturing the essential aspects of language-integrated querying using effects in Links and quotation in LINQ. We show via translations from Eff to Quot and back that the two approaches are equivalent in expressiveness. Based on the translation from Eff to Quot, we extend a simple Links compiler to handle queries.

==> fig-effsub-typing.tex <==
\begin{figure*}

\begin{smathpar}
  \boxed{\Gamma \vdash M : A \eff E}\qquad \boxed{E_1 \leq E_2} \hfill \\
  \inferrule[Var] { } {\Gamma, x:A \vdash x : A \eff E}
%
\and
%
  \inferrule[Const] {\Sigma(c) = A} {\Gamma \vdash c : A \eff E}
%
\and
%
  \inferrule[Op]
  {\Sigma(\op) = (\overline{O}) \to O \\
    \overline{\Gamma \vdash M : O \eff E}} {\Gamma \vdash
    \op(\overline{M}) : O \eff E}
%
\and
%
  \inferrule[Lam] {\Gamma, x:A \vdash M : B \eff E} {\Gamma \vdash
    \lambda^E x^A.M:A \TO{E} B \eff E'}
%
\and
%
  \inferrule[App] {\Gamma \vdash M : A \TO{E'} B \eff E \\ \Gamma
    \vdash N : A \eff E \\ E' \leq E} {\Gamma \vdash M~N : B \eff E}
%
\and
%
  \inferrule[If]
  {\Gamma \vdash L : \Bool \eff E\\
    \Gamma \vdash M : \tColl{A} \eff E} {\Gamma \vdash \If\,L\,M : \tColl{A} \eff
    E}
%
\and
%
  \inferrule[Record] {\overline{\Gamma \vdash M : A \eff E}} {\Gamma
    \vdash \record{\overline{\ell=M}} : \record{\overline{\ell:A}} \eff E}
%
\and
%
  \inferrule[Project] {\Gamma \vdash M : \record{\overline{\ell:A}}
    \eff E} {\Gamma \vdash M.{\ell_i} : A_i \eff E}
%
\and
%
  \inferrule[Empty] { } {\Gamma \vdash \zero : \tColl{A} \eff E}
%
\and
%
  \inferrule[Singleton] {\Gamma \vdash M : A \eff E} {\Gamma \vdash
    \singleton{M} : \tColl{A} \eff E}
%
\and
%
  \inferrule[Union] {\Gamma \vdash M : \tColl{A} \eff E \\ \Gamma \vdash
    N : \tColl{A} \eff E} {\Gamma \vdash M \plus N : \tColl{A} \eff E}
%
\and
%
  \inferrule[For]
  {\Gamma \vdash M : \tColl{A} \eff E \\
    \Gamma,x:A \vdash N : \tColl{B} \eff E} {\Gamma \vdash \For\,(x^A
    \gets M)\,N : \tColl{B} \eff E}
  %
\and
%
  \inferrule[Table] {\Sigma(t) = \tColl{A}} {\Gamma \vdash \Table~t :
    \tColl{A} \eff \db}
%
\and
%
  \inferrule[Query] {\Gamma \vdash M : \tColl{R} \eff \db} {\Gamma
    \vdash \Query~M : \tColl{R} \eff \pl}
%
\and
%
%%   \inferrule[Upcast] {\Gamma \vdash M : A \eff E_1 \\ E_1 \leq E_2}
%%   {\Gamma \vdash M : A \eff E_2}
%% %
%% \and
%
  \inferrule[Rec] {\Gamma,f:A \TO{\pl} B,x:A \vdash M : B \eff \pl}
  {\Gamma \vdash \rec{f^{A \TO{\pl} B}}{x^A}{M} : A \TO{\pl} B \eff E}
%
\and
%
  \inferrule[Fold]
  {\Gamma \vdash L : \tColl{A} \eff \pl \\
    \Gamma \vdash M : B \eff \pl \\
    \Gamma \vdash N : A \TO{\pl} B \TO{\pl} B \eff \pl} {\Gamma \vdash
    \fold~L~M~N : B \eff \pl}
\and
  \inferrule[Reflexivity] { } {E \leq E}
%
\and
%
  \inferrule[AnyPl] { } {\any \leq \pl}
%
\and
%
  \inferrule[AnyDb] { } {\any \leq \db}
\end{smathpar}
\caption{\label{fig:eff-typing}Typing and Subeffecting Rules for
  $\EffSub$}
\end{figure*}


==> fig-quot-typing.tex <==
\begin{figure*}

\begin{smathpar}
  \boxed{\Gamma \vdash M : A}\hfill \\

  \inferrule[Var] { } {\Gamma, x:A \vdash x : A}
%
\and
%
  \inferrule[Const] {\Sigma(c) = A} {\Gamma \vdash c : A}
%
\and
%
  \inferrule[Op]
  {\Sigma(\op) = (\overline{O}) \to O \\
    \overline{\Gamma \vdash M_i : O_i}} {\Gamma \vdash \op(\overline{M}) : O}
%
\and
%
  \inferrule[Lift] {\Gamma \vdash M : O} {\Gamma \vdash
    \lift{M} : \tQuote{O}}
\and
%
  \inferrule[Lam] {\Gamma, x:A \vdash M : B} {\Gamma \vdash \lambda
    x^A.M:A \to B}
%
\and
%
  \inferrule[App] {\Gamma \vdash M : A \to B \\ \Gamma \vdash N : A}
  {\Gamma \vdash M~N : B}
%
\and
%
  \inferrule[If]
  {\Gamma \vdash L : \Bool \\
    \Gamma \vdash M : \tColl{A}} {\Gamma \vdash \If\,L\,M : \tColl{A}}
%
\and
%
  \inferrule[Record] {\overline{\Gamma \vdash M : A}} {\Gamma \vdash
    \record{\overline{\ell=M}} : \record{\overline{\ell:A}}}
%
\and
%
  \inferrule[Project] {\Gamma \vdash M : \record{\overline{\ell:A}}}
  {\Gamma \vdash M.{\ell_i} : A_i}
%
\and
%
  \inferrule[Empty] { } {\Gamma \vdash \zero : \tColl{A}}
%
\and
%
  \inferrule[Singleton] {\Gamma \vdash M : A} {\Gamma \vdash
    \singleton{M} : \tColl{A}}
%
\and
%
  \inferrule[Union] {\Gamma \vdash M : \tColl{A} \\ \Gamma \vdash N :
    \tColl{A}} {\Gamma \vdash M \plus N : \tColl{A}}
%
\and
%
  \inferrule[For]
  {\Gamma \vdash M : \tColl{A} \\
    \Gamma,x:A \vdash N : \tColl{B}} {\Gamma \vdash \For\,(x \gets M)\,N
    : \tColl{B}}
%
\and
%
  \inferrule[Quote] {\Gamma; \cdot \vdash M : A} {\Gamma \vdash
    \Quote{M} : \tQuote{A}}
%
\and
%
  \inferrule[Query] {\Gamma \vdash M : \tQuote{\tColl{R}}}
  {\Gamma \vdash \Query~M : \tColl{R}}
%
\and
%
  \inferrule[Rec] {\Gamma,f:A \to B,x:A \vdash M : B} {\Gamma \vdash
    \rec{f^{A \to B}}{x^A}{M} : A \to B}
%
\and
%
  \inferrule[Fold]
  {\Gamma \vdash L : \tColl{A} \\
    \Gamma \vdash M : B \\
    \Gamma \vdash N : A \to B \to B} {\Gamma \vdash \fold~L~M~N : B}
  \\
  \boxed{\Gamma; \Delta \vdash M : A} \hfill \\
  \inferrule[VarQ] { } {\Gamma; \Delta, x:A \vdash x : A}
%
\and
%
  \inferrule[ConstQ] {\Sigma(c) = A} {\Gamma; \Delta \vdash c : A}
%
\and
%
  \inferrule[OpQ]
  {\Sigma(\op) = (\overline{O}) \to O \\
    \overline{\Gamma; \Delta \vdash M : O}} {\Gamma; \Delta \vdash
    \op(\overline{M}) : O}
%
\and
%
  \inferrule[LamQ] {\Gamma; \Delta, x:A \vdash M : B} {\Gamma; \Delta
    \vdash \lambda x^A.M:A \to B}
%
\and
%
  \inferrule[AppQ] {\Gamma; \Delta \vdash M : A \to B \\ \Gamma;
    \Delta \vdash N : A} {\Gamma; \Delta \vdash M~N : B}
%
\and
%
  \inferrule[IfQ]
  {\Gamma; \Delta \vdash L : \Bool \\
    \Gamma; \Delta \vdash M : A \\
    \Gamma; \Delta \vdash N : A} {\Gamma; \Delta \vdash \If\,L\,M\,N :
    A}
%
\and
%
  \inferrule[RecordQ] {\overline{\Gamma; \Delta \vdash M : A}}
  {\Gamma;\Delta \vdash \record{\overline{\ell=M}} :
    \record{\overline{\ell:A}}}
%
\and
%
  \inferrule[ProjectQ] {\Gamma; \Delta \vdash M :
    \record{\overline{\ell:A}}} {\Gamma; \Delta \vdash M.{\ell_i} :
    A_i}
%
\and
%
  \inferrule[EmptyQ] { } {\Gamma; \Delta \vdash \zero^A : \tColl{A}}
%
\and
%
  \inferrule[SingletonQ] {\Gamma; \Delta \vdash M : A} {\Gamma; \Delta
    \vdash \singleton{M} : \tColl{A}}
%
\and
%
  \inferrule[UnionQ] {\Gamma;\Delta \vdash M : \tColl{A} \\ \Gamma;\Delta \vdash N :
    \tColl{A}} {\Gamma;\Delta \vdash M \plus N : \tColl{A}}
%
\and
%
  \inferrule[ForQ]
  {\Gamma; \Delta \vdash M : \tColl{A} \\
    \Gamma; \Delta, x:A \vdash N : \tColl{B}} {\Gamma; \Delta \vdash
    \For\,(x \gets M)\,N : \tColl{B}}
%
\and
%
  \inferrule[Table] {\Sigma(t) = \tColl{R}} {\Gamma; \Delta \vdash
    \Table~t : \tColl{R}}
%
\and
%
  \inferrule[Antiquote] {\Gamma \vdash M : \tQuote{A}}
  {\Gamma; \Delta \vdash \AntiQuote{M} : A}
\end{smathpar}
\caption{\label{fig:quot-typing}Typing Rules for $\Quot$}
\end{figure*}


==> macros.tex <==
\newenvironment{round}
  {\begin{tikzpicture}[baseline={([yshift={-\ht\strutbox}]current bounding box.west)},
                    outer sep=0pt,inner sep=0pt]}
  {\draw [rounded corners=.5em] (table.north west) rectangle (table.south east);
   \end{tikzpicture}}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}

\newcommand{\sam}[1]{{\color{red} [\textbf{Sam:} #1]}}
\newcommand{\james}[1]{{\color{red} [\textbf{James:} #1]}}

\definecolor{shade}{RGB}{223,223,223}
\newcommand\shade[1]{\setlength{\fboxsep}{0pt}\colorbox{shade}{\ensuremath{#1}}}
%\newcommand{\shade}[1]{\colorbox{shade}{\ensuremath{#1}}}

\newcommand\shaderow{\noalign{\vskip-0.4pt}\rowcolor{shade}}

\newcommand{\trsim}{\lesssim}
\newcommand{\trbisim}{\eqsim}

%%% Gabriel's macros

\newcommand\mysc[1]{{\rmfamily\textsc{#1}}\xspace}
\newcommand\links{\mysc{Links}}
\newcommand\sql{\mysc{SQL}}
\newcommand\js{\mysc{Javascript}}
\newcommand\ocaml{\mysc{Ocaml}}

\newcommand\refsec[1]{\hyperref[#1]{section \ref*{#1}}}


\lstdefinelanguage{links}{
  morekeywords={var,for},
  otherkeywords={<-,<--,=},
  morekeywords=[2]{table,database,with,from},
  classoffset=0,
  morestring=[b]"
}


\lstset{
  tabsize=4,
  basicstyle=\ttfamily\scriptsize,
  % upquote=true,
  aboveskip={0.5\baselineskip},
  columns=fixed,
  showstringspaces=false,
  extendedchars=true,
  breaklines=true,
  prebreak = \raisebox{0ex}[0ex][0ex]{\ensuremath{\hookleftarrow}},
  showtabs=false,
  showspaces=false,
  showstringspaces=false,
  identifierstyle=,
  keywordstyle=\color[rgb]{0.1,0.1,0.7},
  keywordstyle=[2]\color[rgb]{0.1,0.6,0.1},
  commentstyle=\color[rgb]{0.133,0.545,0.133},
  stringstyle=\color[rgb]{0.727,0.326,0.2},
}

\newcommand\sig[1]{{\tt #1}}
\newcommand\mycode[1]{{\tt #1}}
\newcommand\linkslst[1]{\lstinputlisting[language=links]{#1}}
\newcommand\effect[1]{{\em #1}}

\newcommand\ocamlc[1]{\lstinline[language={[Objective]Caml},basicstyle=\ttfamily\normalsize]{#1}}

\newcommand\module[1]{{\bf #1}}

%comment inside bnf
\renewcommand\comment[1]{{\color{gray} $//$ #1}}

\newcommand{\todo}[1]{[\textbf{TODO: } #1 ]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\blue}[1]{#1}
\newcommand{\red}[1]{#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bl}{~}

\newcommand{\key}[1]{\textsf{#1}}
\newcommand{\fld}[1]{\key{#1}}
\newcommand{\var}[1]{\mathit{#1}}
\newcommand{\str}[1]{\textsf{``#1''}}
\newcommand{\bag}[1]{\collection{#1}}

\newcommand{\ampersand}{\mathbin{\textsf{\&}}}

\newcommand{\blist}{\begin{array}[t]{@{}l@{}}}
\newcommand{\elist}{\end{array}}

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\lceil #1 \rceil}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\labels}{\mathit{labels}}

\newcommand{\CC}{\mathcal{C}}
\newcommand{\EC}{\mathcal{E}}
\newcommand{\QC}{\mathcal{Q}}
\newcommand{\SC}{\mathcal{S}}

\newcommand{\set}[1]{\{{#1}\}}
\newcommand{\sem}[1]{\llbracket{#1}\rrbracket}

\newcommand{\FV}{\mathit{FV}}
\newcommand{\FTV}{\mathit{FTV}}
\newcommand{\FEV}{\mathit{FEV}}
\newcommand{\recName}{\mathsf{rec}}
\newcommand{\rec}[3]{\recName~{#1}~{#2}.{#3}}

\newcommand{\Int}{\mathit{Int}}
\newcommand{\Bool}{\mathit{Bool}}
\newcommand{\String}{\mathit{String}}
%\newcommand{\Coll}{\mathit{List}}
%\newcommand{\Coll}{\mathit{Bag}}

\newcommand{\Exp}{\mathit{Exp}}
\newcommand{\Const}{\mathit{Const}}

\newcommand{\recordl}{\langle}
\newcommand{\recordr}{\rangle}
\newcommand{\record}[1]{\recordl {#1} \recordr}
\newcommand{\tuple}{\record}
%\newcommand{\collection}[1]{\texttt{[} {#1} \texttt{]}}
\newcommand{\collection}[1]{\mathopen{\texttt{[}} {#1} \mathclose{\texttt{]}}}
\newcommand{\singleton}[1]{\ret{#1}} %\collection{#1}}
%\newcommand{\Concat}{\mathsf{concat}}
%\newcommand{\Concat}{\biguplus}
\newcommand{\concat}{\mathbin{+\!\!+}}
%\newcommand{\concat}{\uplus}

\newcommand{\Database}{\mathsf{database}}
\newcommand{\Query}{\mathsf{query}}
\newcommand{\Var}{\mathsf{var}}
\newcommand{\Type}{\mathsf{type}}

\newcommand{\Expression}[1]{\mathit{Expression}\mathopen{<}#1\mathclose{>}}
\newcommand{\IQueryable}[1]{\mathit{IQueryable}\mathopen{<}#1\mathclose{>}}
\newcommand{\IEnumerable}[1]{\mathit{IEnumberable}\mathopen{<}#1\mathclose{>}}
\newcommand{\IEnumerator}[1]{\mathit{IEnumerator}\mathopen{<}#1\mathclose{>}}
\newcommand{\Func}[2]{\mathit{Func}\mathopen{<}#1,#2\mathclose{>}}

\newcommand{\Expr}[1]{\mathit{Expr}(#1)}

\newcommand{\Lift}{\mathsf{lift}}
\newcommand{\Return}{\mathsf{return}}
\newcommand{\Empty}{\mathsf{empty}}

%% \newcommand{\retl}{\Return\,(}
%% \newcommand{\retr}{)}
%% \newcommand{\ret}[1]{\Return\,{#1}}

\newcommand{\retl}{\texttt{[}}
\newcommand{\retr}{\texttt{]}}
\newcommand{\ret}[1]{\retl{#1}\retr}


\newcommand{\lam}[1]{\lambda #1.\,}

\renewcommand{\plus}{\concat}
\newcommand{\zero}{\texttt{[]}}

\newcommand{\Case}{\mathsf{case}}
\newcommand{\Of}{\mathsf{of}}

\newcommand{\Let}{\mathsf{let}}
\newcommand{\In}{\mathsf{in}}

\newcommand{\gives}{\Rightarrow}

\newcommand{\TableType}{\mathit{Table}}
\newcommand{\Table}{\mathsf{table}}

\newcommand{\For}{\mathsf{for}}
\newcommand{\If}{\mathsf{if}}
\newcommand{\Then}{\mathsf{then}}
\newcommand{\Else}{\mathsf{else}}

\newcommand{\Where}{\mathsf{where}}

\newcommand{\With}{\mathsf{with}}

\newcommand{\True}{\mathsf{true}}
\newcommand{\False}{\mathsf{false}}

\newcommand{\Quote}[1]{\mathopen{\texttt{<@}~} {#1} \mathclose{~\texttt{@>}}}
\newcommand{\AntiQuote}[1]{\texttt{(\%}{#1}\texttt{)}}


% effects
\newcommand{\eff}{\mathbin{!}}

\newcommand{\TO}[1]{\to^{#1}}

\newcommand{\db}{\mathbf{db}}
\newcommand{\pl}{\mathbf{pl}}
\newcommand{\any}{\mathbf{any}}

\newcommand{\evar}{\varepsilon}

%% \newcommand{\toDb}{\mathord{\uparrow}_{\db}}
%% \newcommand{\toPl}{\mathord{\uparrow}_{\pl}}

\newcommand{\atName}{\uparrow}
\newcommand{\at}[2]{{#1}\uparrow{#2}}
\newcommand{\atDb}[1]{\at{#1}{\db}}
\newcommand{\atPl}[1]{\at{#1}{\pl}}

\newcommand{\AtName}{\star}
\newcommand{\At}[2]{{#1}\AtName{#2}}

\newcommand{\envAt}[2]{\sem{#1}_{#2}}

%\newcommand{\lookup}[4]{{#1}^{#3} \mathbin{@_{#2}} #4}
\newcommand{\lookup}[3]{{#1} \mathbin{@_{#2}} #3}


\newcommand{\op}{\mathit{op}}
\newcommand{\opdelta}{\delta}

\newcommand{\abs}{\circ}
\newcommand{\pre}{\bullet}

% quotation
%% \newcommand{\cQuote}[2]{\mathop{\blacktriangleright_{#1}}{#2}}
%% \newcommand{\cAntiquote}[2]{\mathop{\blacktriangleleft_{#1}}{#2}}
%% \newcommand{\cQuoted}[2]{\mathop{\vartriangleright_{#1}}{#2}}
\newcommand{\tQuote}[1]{\mathsf{Expr}\mathopen{\texttt{<}}\,{#1}\,\mathclose{\texttt{>}}}
  % \mathsf{Exp}\langle #1 \rangle}
\newcommand{\tColl}[1]{\texttt{[}#1\texttt{]}}

%\newcommand{\cQuote}[2]{\lceil {#2} \rceil_{#1}}
%\newcommand{\cAntiquote}[2]{\lfloor {#2} \rfloor_{#1}}
%\newcommand{\cQuoted}[2]{{#1} \mathbin{\blacktriangleright} {#2}}

%\newcommand{\eQuote}[2]{\mathopen{\lceil} {#1} \mathclose{\rceil}^{#2}}
%\newcommand{\eQuoted}[2]{{#1} \mathbin{\blacktriangleright} {#2}}

%\newcommand{\eQuoteC}[1]{\mathopen{\texttt{<@}~} {#1} \mathclose{~\texttt{@>}}}
%\newcommand{\eAntiquote}[1]{\texttt{(\%}{#1}\texttt{)}}
%\newcommand{\eQuotedC}[1]{\mathop{\blacktriangleright} {#1}}



\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}

\newenvironment{mysyntax}{\[\ba{@{}l@{~~}l@{~}c@{~}l@{}}}{\ea\]}
\newenvironment{laws}{\[\ba{l@{}r@{~~}c@{~~}l}}{\ea\]}
\newenvironment{equations}{\[\ba{r@{~~}c@{~~}l@{\quad}l}}{\ea\]}

\newenvironment{iequations}{\ba[t]{r@{~~}c@{~~}l@{\quad}l}}{\ea}

% syntactic category
\newcommand{\cat}[1]{\text{({#1})}}


\newcommand{\TLINQ}{T-LINQ\xspace}

\newcommand{\Quot}{\mathsf{Quot}}
\newcommand{\QuotVar}{\mathsf{Quot}'}
\newcommand{\Eff}{\mathsf{Eff}}
\newcommand{\PolyEff}{\mathsf{PolyEff}}
\newcommand{\EffSub}{\mathsf{Eff_{\leq}}}

\newcommand{\QuotClosed}{\mathsf{Quot}_{\square}}


% translations
\newcommand{\dup}[1]{\langlebar{#1}\ranglebar}

\newcommand{\dupEff}[2]{\langlebar{#1}\ranglebar_{#2}}
\newcommand{\dupX}[1]{\dupEff{#1}{X}}
\newcommand{\dupY}[1]{\dupEff{#1}{Y}}
\newcommand{\duppl}[1]{\dupEff{#1}{\pl}}
\newcommand{\dupdb}[1]{\dupEff{#1}{\db}}

\newcommand{\trans}[1]{\sem{#1}}
\newcommand{\untrans}[1]{\llparenthesis{#1}\rrparenthesis}

\newcommand{\untransX}[1]{\untrans{#1}_X}
\newcommand{\untranspl}[1]{\untrans{#1}_{\pl}}
\newcommand{\untransdb}[1]{\untrans{#1}_{\db}}

\newcommand{\untransq}[3]{\untransdb{#1}^{{#2},{#3}}}
\newcommand{\envTy}[1]{\mathit{typeof}(#1)}


%% % constructors
%% \newcommand{\kLeft}{\mathrm{Left}}
%% \newcommand{\kRight}{\mathrm{Right}}

%% \newcommand{\kConst}{\mathrm{Const}}
%% \newcommand{\kVar}{\mathrm{Var}}
%% \newcommand{\kInt}{\mathrm{Int}}
%% \newcommand{\kBool}{\mathrm{Bool}}
%% \newcommand{\kString}{\mathrm{String}}
%% \newcommand{\kLam}{\mathrm{Lam}}
%% \newcommand{\kApp}{\mathrm{App}}
%% \newcommand{\kRecord}{\mathrm{Record}}
%% \newcommand{\kSingleton}{\mathrm{Singleton}}
%% \newcommand{\kFor}{\mathrm{For}}
%% \newcommand{\kConcat}{\mathrm{Concat}}
%% \newcommand{\kIf}{\mathrm{If}}
%% \newcommand{\kProj}{\mathrm{Proj}}
%% \newcommand{\kTable}{\mathrm{Table}}
%% \newcommand{\kList}{\mathrm{List}}

% operational semantics
\newcommand{\evalto}{\longrightarrow}

\newcommand{\rewriteto}{\leadsto}
\newcommand{\adhocto}{\hookrightarrow}

\newcommand{\theDb}{\var{db}}
\newcommand{\DB}{\Omega}

% normalisation
\newcommand{\norm}{\mathit{norm}}
\newcommand{\normEff}[1]{|#1|}
\newcommand{\normQuot}[1]{\|#1\|}

\newcommand{\eval}{\mathit{eval}}

\newcommand{\substTables}{\mathit{substTables}}

\newcommand{\Split}[2]{\mathit{split}_{#1}({#2})}
\newcommand{\Splitl}[1]{\Split{\vec{\ell}}{#1}}
\newcommand{\Splitnl}[1]{\mathopen{\parallel}{#1}\mathclose{\parallel}}

\newcommand{\reify}{\mathord{\downarrow}}

% splicing constructors
\newcommand{\dbInt}{\mathsf{Int}}
\newcommand{\dbBool}{\mathsf{Bool}}
\newcommand{\dbString}{\mathsf{String}}

%\newcommand{\lift}{\mathsf{Base}}
\newcommand{\lift}[1]{\Lift~{#1}}
%\newcommand{\dbColl}{\mathsf{List}}
\newcommand{\dbColl}{\mathsf{Bag}}

\newcommand{\fold}{\mathsf{fold}}

\newcommand{\transX}[1]{\trans{#1}_X}
\newcommand{\transpl}[1]{\trans{#1}_\pl}
\newcommand{\transdb}[1]{\trans{#1}_{\db{\vphantom{\any}}}}

\newcommand{\transXr}[1]{\transX{#1}^\rho}
\newcommand{\transplr}[1]{\transpl{#1}^\rho}
\newcommand{\transdbr}[1]{\transdb{#1}^\rho}

\newcommand{\error}{\mathit{error}}

% record extension
\newcommand{\extend}{\mathit{extend}}

% indexing
\newcommand{\xtoy}[2]{_{{#1}=1}^{#2}}
\newcommand{\iton}{\xtoy{i}{n}}
\newcommand{\jtom}{\xtoy{j}{m}}


\newcommand{\evaltoeff}[1]{\mathbin{\evalto}} %_{#1}}}
\newcommand{\evaltoX}{\evaltoeff{X}}
\newcommand{\evaltodb}{\evaltoeff{\db}}
\newcommand{\evaltopl}{\evaltoeff{\pl}}


\newenvironment{nop}{}{}
\newenvironment{smathpar}{
\begin{nop}\small\begin{mathpar}}{
\end{mathpar}\end{nop}\ignorespacesafterend}

%doubling
% \newcommand{\dupp}[1]{\dup{(#1)}}
% \newcommand{\dupXp}[1]{\dupX{(#1)}}
% \newcommand{\dupYp}[1]{\dupY{(#1)}}
% \newcommand{\dupplp}[1]{\duppl{(#1)}}
% \newcommand{\dupdbp}[1]{\dupdb{(#1)}}

\newcommand{\lambdaNRC}{\lambda^{\mathrm{NRC}}}

\newcommand{\ltoo}[1]{\stackrel{#1}{\longrightarrow}}
\newcommand{\lToo}[1]{\stackrel{#1}{\Longrightarrow}}
\newcommand{\Too}{\Longrightarrow}
\newcommand{\too}{\longrightarrow}

\newcommand{\unit}{{\record{}}}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "links-compile"
%%% End: 

